How to Attain Communication-Efficient DNN Training? Convert, Compress, Correct

This paper introduces CO3 -- an algorithm for communication-efficient federated Deep Neural Network (DNN) training. CO3 takes its name from three processing applied which reduce the communication load when transmitting the local DNN gradients from the remote users to the Parameter Server. Namely: (i) gradient quantization through floating-point conversion, (ii) lossless compression of the quantized gradient, and (iii) quantization error correction. We carefully design each of the steps above to assure good training performance under a constraint on the communication rate. In particular, in steps (i) and (ii), we adopt the assumption that DNN gradients are distributed according to a generalized normal distribution, which is validated numerically in the paper. For step (iii), we utilize an error feedback with memory decay mechanism to correct the quantization error introduced in step (i). We argue that the memory decay coefficient, similarly to the learning rate, can be optimally tuned to improve convergence. A rigorous convergence analysis of the proposed CO3 with SGD is provided. Moreover, with extensive simulations, we show that CO3 offers improved performance when compared with existing gradient compression schemes in the literature which employ sketching and non-uniform quantization of the local gradients.

==> theoretical_proof.tex <==
\section{Convergence Proof}
\label{sec:Theoritical proof}
\textcolor{blue}{In this section, we explore the upper bound of the optimal gap of SGD as well as the variance of the optimal gap when modelling the stochastic gradient as a $\gennorm$ distribution. 
%
By analyzing these bounds, we can gain insight into the convergence of SGD. To demonstrate this convergence, we follow the steps outlined in the book\cite{shalev2014understanding} and provide a rigorous proof. 
%
Specifically, we carefully examine the properties of the gennorm distribution and leverage them to derive the upper bound. 
%
By doing so, we can demonstrate the effectiveness of SGD in minimizing the objective function and achieving convergence in the optimization process.}

\subsection{SGD optimal gap}
\textcolor{blue}{The Lemma 1 is from Lemma 14.1 of the book \cite{shalev2014understanding}.}
\newtheorem{lemma}{Lemma}
\begin{lemma}
Let $v_1,...,v_T$ be an arbitrary sequence of vectors. Any algorithm with an initialization $w^{(1)}=0$ and an update rule of the form
    \begin{align}
        w^{(t+1)}=w^{(t)}-\eta v_t
    \end{align}
satisfies
    \begin{align}
        \sum_{t=1}^{T}<w^{(t)}-w^*,v_t> \leq \frac{{||w^*||}^2}{2\eta}+\frac{\eta}{2}\sum_{t=1}^{T}{||v_t||}^2
    \end{align}
\end{lemma}


Let f be a convex function and let $w^*\in \mathop{\arg\min}_{w:||w||\leq B}f(w)$
\begin{align}
    f(\Bar{w})-f(w^*)&=f(\frac{1}{T}\sum_{t=1}^{T}w^{(t)})-f(w^*)\\
    &\leq \frac{1}{T}\sum_{t=1}^{T}(f(w^{(t)}))-f(w^*)\\
    &= \frac{1}{T}\sum_{t=1}^{T}(f(w^{(t)})-f(w^*))
\end{align}

\newtheorem{theorem}{Theorem}
\begin{theorem}
    The SGD optimal gap is 
        \begin{align}
            \mathbb{E}_{v_{1:T}}[f(\Bar{w})-f(w^*)]\leq \frac{{||w^*||}^2}{2\eta T}+\frac{\eta}{2T}\sum_{t=1}^{T}\sigma_t^2
        \end{align}
    proof:
        Taking expectation of equation (16)
        \begin{align}
            \mathbb{E}_{v_{1:T}}[f(\Bar{w})-f(w^*)] \leq \mathbb{E}_{v_{1:T}}[\frac{1}{T}\sum_{t=1}^{T}(f(w^{(t)})-f(w^*))]
        \end{align}
        Taking expectation of equation (13)
        \begin{align}
            \mathbb{E}_{v_{1:T}}[\frac{1}{T}\sum_{t=1}^{T}<w^{(t)}-w^*,v_t>] &\leq \mathbb{E}_{v_{1:T}}[\frac{{||w^*||}^2}{2\etaT}+\frac{\eta}{2T}\sum_{t=1}^{T}{||v_t||}^2]\\
            &= \frac{{||w^*||}^2}{2\eta T}+\frac{\eta}{2T}\sum_{t=1}^{T}\mathbb{E}_{v_{1:T}}[{||v_t||}^2]\\
            &= \frac{{||w^*||}^2}{2\eta T}+\frac{\eta}{2T}\sum_{t=1}^{T}\sigma_t^2
        \end{align}
        It is left to show that
        \begin{align}
            \mathbb{E}_{v_{1:T}}[\frac{1}{T}\sum_{t=1}^{T}(f(w^{(t)})-f(w^*))]\leq\mathbb{E}_{v_{1:T}}[\frac{1}{T}\sum_{t=1}^{T}<w^{(t)}-w^*,v_t>]
        \end{align}
        \begin{align}
            \mathbb{E}_{v_{1:T}}[<w^{(t)}-w^*,v_t>]&= \mathbb{E}_{v_{1:t}}[<w^{(t)}-w^*,v_t>]\\
            &= \mathbb{E}_{v_{1:t-1}}\mathbb{E}_{v_{1:t}}[<w^{(t)}-w^*,v_t>|v_{1:t-1}]\\
            &= \mathbb{E}_{v_{1:t-1}}[<w^{(t)}-w^*,\mathbb{E}_{v_t}[v_t|v_{1:t-1}]>]
        \end{align}
        Since $w^{(t)}$ only depends on $v_{1:t-1}$ and SGD requires that $\mathbb{E}_{v_t}[v_t|w^{(t)}] \in \partial f(w^{(t)})$
        \begin{align}
            \mathbb{E}_{v_{1:t-1}}[<w^{(t)}-w^*,\mathbb{E}_{v_t}[v_t|v_{1:t-1}]>]\geq \mathbb{E}_{v_{1:t-1}}[f(w^{(t)})-f(w^*)]
        \end{align}
        Overall,
        \begin{align}
            \mathbb{E}_{v_{1:T}}[<w^{(t)}-w^*,v_t>] &\geq \mathbb{E}_{v_{1:t-1}}[f(w^{(t)})-f(w^*)]\\
            &= \mathbb{E}_{v_{1:T}}[f(w^{(t)})-f(w^*)]
        \end{align}
        Summing over t, dividing by T, and using the linearity of expectation, we get
        that Equation (11) holds, which concludes the proof.
\end{theorem}
\textcolor{blue}{From Theorem1, the upper bound is consist of norm square of optimal solution and  the summation of gradient variance of each step. When we assume the gradient as $\gennorm$ distribution with mean $0$ and bounded variance, the convergence is guaranteed. This bound provides important insight into the convergence behavior of SGD under $\gennorm$ assumption.}
\subsection{Variance of SGD optimal gap}
\begin{theorem}
    The variance of SGD optimal gap
    \begin{align}
        var(f(\Bar{w})-f(w^*)) &= \mathbb{E}_{v_{1:T}}[{(f(\Bar{w})-f(w^*))}^2]-{(\mathbb{E}_{v_{1:T}}[f(\Bar{w})-f(w^*)])}^2\\
        &\leq \mathbb{E}_{v_{1:T}}[{(f(\Bar{w})-f(w^*))}^2]
    \end{align}
    
    First,
    \begin{align}
        {(f(\Bar{w})-f(w^*))}^2 &\leq {(\frac{1}{T}\sum_{t=1}^{T}(f(w^{(t)})-f(w^*)))}^2\\
        &\leq\frac{1}{T^2}(T\sum_{t=1}^T{(f(w^{(t)})-f(w^*))}^2)\\
        &=\frac{1}{T}\sum_{t=1}^{T}{(f(w^{(t)})-f(w^*))}^2
    \end{align}
    
    Taking expectation of equation (33)
    \begin{align}
        \mathbb{E}_{v_{1:T}}[{(f(\Bar{w})-f(w^*))}^2] &= \frac{1}{T}\sum_{t=1}^{T}\mathbb{E}_{v_{1:T}}[{(f(w^{(t)})-f(w^*))}^2]\\
        &\leq \frac{1}{T}\sum_{t=1}^{T}\mathbb{E}_{v_{1:T}}[{(\rho||w^{(t)}-w^*||)}^2]\\
        &=\frac{\rho^2}{T}\sum_{t=1}^{T}\mathbb{E}_{v_{1:T}}[{||w^{(t)}-w^*||}^2]
    \end{align}
    The equation (35) is derived by the assumption that the gradient is $\rho$-Lipschitz continuous.
    
    \begin{align}
        \mathbb{E}_{v_{1:t}}[{||w^{(t)}-w^*||}^2] &= \mathbb{E}_{v_{1:t-1}}[{||w^{(t-1)}-w^*||}^2] -2\eta{(w^{(t-1)}-w^*)}^T\mathbb{E}_{v_{t}}v_t+\eta^2\mathbb{E}_{v_{t}}{||v_t||}^2
    \end{align}
    Assume that the stochastic gradients $v_t$ follow the GenNorm distribution with mean 0, variance $\sigma_t^2$
    \begin{align}
        \mathbb{E}_{v_{1:t}}[{||w^{(t)}-w^*||}^2] &= \mathbb{E}_{v_{1:t-1}}[{||w^{(t-1)}-w^*||}^2] +\eta^2\sigma_t^2\\
        &={||w^*||}^2 + \eta^2\sum_{t=1}^{T}\sigma_t^2
    \end{align}
    
    Substitute equation (39) into equation (36)
    \begin{align}
        \mathbb{E}_{v_{1:T}}[{(f(\Bar{w})-f(w^*))}^2] &\leq \frac{\rho^2}{T}\sum_{t=1}^{T}\mathbb{E}_{v_{1:T}}[{||w^{(t)}-w^*||}^2]\\
        &=\frac{\rho^2}{T}\sum_{t=1}^{T}({||w^*||}^2 + \eta^2\sum_{t=1}^{T}\sigma_t^2)\\
        &=\rho^2{||w^*||}^2+\rho^2\eta^2\sum_{t=1}^{T}\sigma_t^2
    \end{align}
    
\end{theorem}
